Whose Knowledge is Valued?: Epistemic Injustice in CSCW Applications

Social computing scholars have long known that people do not interact with knowledge in straightforward ways, especially in digital environments. While policies around knowledge are essential for targeting misinformation, they are value-laden; in choosing how to present information, we undermine non-traditional -- often non-Western -- ways of knowing. Epistemic injustice is the systemic exclusion of certain people and methods from the knowledge canon. Epistemic injustice chips away at one's testimony and vocabulary until they are stripped of their due right to know and understand. In this paper, we articulate how epistemic injustice in sociotechnical applications leads to material harm. Inspired by a hybrid collaborative autoethnography of 14 CSCW practitioners, we present three cases of epistemic injustice in sociotechnical applications: online transgender healthcare, identity sensemaking on r/bisexual, and Indigenous ways of knowing on r/AskHistorians. We further explore signature tensions across our autoethnographic materials and relate them to previous CSCW research areas and personal non-technological experiences. We argue that epistemic injustice can serve as a unifying and intersectional lens for CSCW research by surfacing dimensions of epistemic community and power. Finally, we present a call to action of three changes the CSCW community should make to move toward its own goals of research justice. We call for CSCW researchers to center individual experiences, bolster communities, and remediate issues of epistemic power as a means towards epistemic justice. In sum, we recount, synthesize, and propose solutions for the various forms of epistemic injustice that CSCW sites of study -- including CSCW itself -- propagate.

==> sections/archive/cases/online-mh-care.tex <==
- mental health care is a hermeneutical resource - It helps people interpret their experiences
- HCI and CSCW have studied technology mediated pathways to mental health care and find it is filled with unjustified frictions (suicidal on a sunday) and steeped in colonialized views of mental health that stigmatize support seekers (online narratives paper) 
- This lack of hermeneutical resources in CSCW applications is epistemic injustice.

==> sections/archive/cases/wikipedia-gender-edit-gap.tex <==
- Wikipedia is a site of knowledge

Now that Wikipedia has existed for 20 years, there have been continuous efforts to make the platform more diverse and inclusive. For example, seminal Wikipedia work has explored the gender-edit gap– the disproportionate amount of male-identifying editors and subjects to gender minorities, such as female or non-binary folks \cite{Houtti2022-uo,Menking2019-ep,Lam2011-up,Hargittai2015-yk}. Since this formative research, there have been numerous examples of trying to redress Wikipedia’s initial lack of diversity and inclusivity, such as edit-a-thons [cite article Isaac sent].

Despite these interventions, and their proven effectiveness [cite],  it is unclear whether Wikipedia is equitable. While anyone can contribute, there are barriers to lasting or repeated contribution on the platform, such as dense policy \cite{Viegas2007-uq}, aggressive edit reversions\cite{Halfaker2011-lp}, and heavy-handed moderation interventions \cite{Ajmani2023-yk}. 

Anticipatory injustice

==> sections/archive/rw.tex <==
\subsection{Knowledge-Production in CSCW}
As a research venue, CSCW has a rich history of studying knowledge production online. Notably, CSCW has been publishing work on Wikipedia for nearly 20 years~\cite{}. Recent work has explored knowledge-based constructs, such as content moderation of misinformation~\cite{}, 

In CSCW specifically,~\citet{Erete2021-xp} invoke epistemic violence to describe their experiences as Black members of the CSCW community. However, other epistemic stances in CSCW are often implicit yet ever-evolving. For example, CSCW used to debate whether Wikipedia can be trusted. Modern Wikipedia discourse presumes the epistemic stance that Wikipedia can be trusted. In this paper, we posit that evolving epistemologies are healthy signs of progress. We specifically highlight one researcher's experience of incorporating Indigenous ways of knowing into their Reddit community. However, this process is ripe with nuance and requires deep interrogation.

\subsection{[Jay?] Data and epistemic injustice}

\subsection{Cases of Epistemic Injustice in CSCW}
\subsubsection{Wikipedia Gender Edit Gap}
\subfile{cases/wikipedia-gender-edit-gap}
\subsubsection{Online Mental Health Care}
\subfile{cases/online-mh-care}




==> sections/archive/taxonomy.tex <==
[NOTE: folks are referenced as "workshop participants" just for the sake of quick drafting, Leah, Jay and Jordan to discuss better verbiage]

In this section we build out a taxonomy of epistemic injustice specifically within CSCW applications based on our collaborative thematic analysis. We suggest that EI can be thought of in three broad categories: contributors, mitigators, and tensions. [FINISH PARAGRAPH]
\subsection{Contributors to Epistemic Injustice}
\begin{tcolorbox}[boxrule=0pt, frame empty]
\begin{itemize}[leftmargin=*]
    \item[] \textbf{Invisibility} of communities and identity groups
    \item[] \textbf{Inaccessibility} of relevant information-rich resources
    \item[] \textbf{Anti-agentic} discourse surrounding knowers
\end{itemize}
\end{tcolorbox}
First, we consider what allows epistemic injustice to take place in CSCW applications. Notably, our participants all agreed that epistemic injustice is not a passive concept: systemic silencing does not "just happen," rather it is an active process that a knowledge community either consciously or unconsciously engages in. This is particularly evidenced by the numerous examples of highly moderated platforms, such as Wikipedia and factual subreddits, that participants raised in their cases. Given that epistemic injustice is active, our participants specifically highlighted design decisions in sociotechnical systems that perpetrate EI.
\subsubsection{(In)visbility} Invisbility is a nuanced construct within epistemic injustice as it is both a \textit{product of} and a \textit{contributor to} EI. Specifically in online communities, EI causes certain stories to never appear within the community. As discussed in the case of Indigenous knowledge within r/AskHistorians, invisibility can be hard to detect and even harder to remediate. 

The invisibility of relevant perspectives and voices is difficult to detect because of what one participant called \textit{failures of existing "evaluations" and "benchmarks"}. For example, Wikipedia has a dizzying amount of policy and governance concerning knowledge on the platform. However, a Wikipedia researcher noted that unfamiliar sources do not always get a fair evaluation.
\begin{quote}
    \textit{``One of Wikipedia's core policies is around Verifiability~\footnote{https://en.wikipedia.org/wiki/Wikipedia:Verifiability}, which, practically speaking, rests on the concept of a reliable source. Whether a source is reliable is a matter of consensus within the editing community but a lot of it relies on familiarity with sources (to be able to judge them). This means that sources that are unknown to the core community can be rejected as non-reliable."}
\end{quote}
In other words, the invisibility of reliable, but non-traditional sources begets further invisibility, causing a vicious cycle of epistemic injustice that goes unchecked [LEAH TO MAYBE ADD A FIGURE?]. The bidirectional relationship between invisibility and epistemic injustice suggests that fact-finding communities, such as Wikipedia and r/AskHistorians, need to view their epistemic stances as dynamic positions rather than static policies. The notion of a reliable source cannot be a one-time stipulation within a community. Rather, as r/AskHistorians suggests, it is an ongoing conversation with those whose voices have been systemically excluded. Our participants noted promising futures of participatory governance designs[cite digital juries] that seek to codify more inclusive forms of knowledge.

However, workshop participants noted that visibility is double-edged sword. In an informationally dense space, such as the internet, curation is necessary. However, participants noted that curation carries its own position on \textit{who and what is deserving of entering the Knowledge cannon.} 

\begin{quote}
This state of affairs directly removes scientifically- and community-validated, high-quality information from the public sphere, and does so specifically for trans people, while other forms of non-formal health advice (e.g., unhealthy body image and exercise influencers, “nutrition” influencers hocking questionable and potentially dangerous supplements, etc) are allowed to freely exist, and even gain traction through algorithmic curation.
\end{quote}

Note that, particularly in algorithmic curation, such as TikTok [cite Ash] and Instagram, it is even easier for these normative stances to go uninterrogated. Previous work has called the TikTok algorithm a ``runaway train.~\cite{Milton2023-vu}" From an epistemic lens, this algorithmic off-the-rails behavior implies that there is little control over who is getting space on the platform and why their information, which ultimately turns into user knowledge, is deserving of that space.

\subsubsection{Inaccessibility}



\subsubsection{Anti-agentic discourse}
Finally, workshop participants reflected inward on discourse within their research communities (CSCW, CHI, FAccT, SIGIR, etc.). Participants noted numerous ways in which language typically associated with raising marginalized identities gets inappropriately wielded, particularly in research settings. We call this ``anti-agentic" discourse: the use of language to discount groups rather than participate with them. Anti-agentic discourse is a form of hermeneutical injustice as misappropriated an interpretive resource (i.e., language). For example, one participant noted that ``at-risk," a term originally used to create more thorough consent procedures in research [cite IRB], \textit{"is thrown around paternalistically in HCI with an exorbitant number of identity groups such as Youth, Queer Folks, Substance Use, Autism/Mental Health, etc."} A researcher in online mental health communities had similar experiences, 
\begin{quote}
\textit{``We need to loosen the idea of what is `normal`, `correct`, or `unsafe` when regarding online mental health communities."}
\end{quote}
They suggested contextual, community-specific approaches to defining these terms in research.

Anti-agentic discourse is particularly problematic in research settings. Researchers are canonically accepted as ``knowers:" people who have the qualities necessary to contribute knowledge. Often in venues, such as CSCW and CHI, we are studying marginalized communities who have deep histories of facing epistemic injustice. Therefore, we, as researchers, must engage with the verbiage of these communities rather than the language that we have passed down through archival research papers.

Self-reflection on the implicit positionalities of researching a historically marginalized community is a promising path forward. To paraphrase~\citet{Braun2006-eg}, researchers cannot simply ‘give voice’ to their participants. As~\citet{Fine1992-ov} argues, even a ‘giving voice’ approach ‘involves carving out unacknowledged pieces of narrative evidence that we select, edit, and deploy to border our arguments’.

% quotes:
%  I have been asked by reviewers to explain how my findings apply to all Bsiexual People. However, this leads to its own sort of epistemic injustice in that bi people  are meant to fit in the neat boxes that HCI reseviewers expect. No such group of bi folks who all think the same exist.  I’ve also received push back for even claiming that there is little research about bi people in HCI (only one study atm in the ACM) because of all the research on LGBTQ+ people generally. The null hypothesis of reviewers is that all queer are the same rather than beginning with differences and having to prove similarities. 



\subsection{Mitigators of EI}
\begin{tcolorbox}[boxrule=0pt, frame empty]
\begin{itemize}[leftmargin=*]
    \item[] \textbf{Prevention} through evaluation and design
    \item[] \textbf{Remediation} of past injustices
    \item[] \textbf{Resistance} to injustices from communities
\end{itemize}
\end{tcolorbox}

\subsection{Tensions of EI}
\begin{tcolorbox}[boxrule=0pt, frame empty]
\begin{itemize}
    \item[] \textbf{Expertise} of contributors
    \item[] \textbf{Gatekeeping} as a necessary component of moderation
    \item[] \textbf{Decentralization}
\end{itemize}
\end{tcolorbox}

\subsubsection{Expertise} In her original work,~\cite{Fricker2007-zh} prefers the term ``knowers" to ``experts" as it distances credibility from large institutions mired in bureaucracy and acontextual demands. However, popular media in the early 2000s questioned whether the internet has created a place where ``suddenly, everyone is an expert."~\footnote{https://www.nytimes.com/2000/02/03/technology/suddenly-everybody-s-an-expert.html} Conceptualizing expertise is particularly important for CSCW research, which has continually explored the harm of rampant misinformation from non-experts [CITE]. However, our workshop participants found that asking \textit{what defines an expert?} demands simultaneously asking \textit{what is the normative position behind defining expertise?}

If created by the community, traditional expertise can help form strong support systems for said community. One participant cited the Transgender Professional Association for Transgender Health (TPATH)~\footnote{https://tpathealth.org/} as an example of traditional experts (e.g., people with medical degrees) creating a community-based knowledge institution. Concisely, TPATH's mission is ``Trans Health by Trans People." Yet, TPATH has had trouble gaining credibility as a collective of medical health experts, particularly in online spaces with algorithmic moderation. Previous work has noted related phenomena where [TAKE FROM WORKSHOP]. As one participant put it, ``in online spaces bodies to formalize knowledge on our own terms are ignored because they are \textit{of} the community, despite the presence of traditional experts"

However, epistemic injustice heavily relies on the continuous interrogation of non-traditional expertise: can someone be a valuable knower without carrying common credentials? This distinction of appropriate level of expertise is especially important when discussing an individual's expertise in their own lived experience. The above case on Trans Health [reference case section] notes that individual experiences are valuable information, but are often sidelined to informal online spaces, such as Reddit. Concerningly, our participants echoed this systemic discounting of their own experience in violent settings. 
\begin{quote}
\textit{``After being robbed at gunpoint while at a friend's home, the police were called, and a less-than-enthusiastic officer arrived to take our statements. I observed that the officer was writing hardly anything down in his notepad despite my rich account of every detail from the color of the gun barrel to the differences in intonation, height, and apparel of the assailants. The cop frequently looked away from me and attempted to restate what I was saying  but with incorrect details."}
\end{quote}

Finally, anticipatory injustice furthers this tension. Gaining traditional expertise requires knowledge that is often inaccessible to outsiders. One participant cited their own struggles with learning about applying to PhD programs. 
\begin{quote}
    \textit{``It wasn’t until after joining as a PhD student that I learned that most successful applicants find their research advisor prior to applying. Information on the department’s website heavily suggests that if you’re interested, you should follow the application process. Contrary to good practice, it does not suggest reaching out to potential research advisors. "}
\end{quote}

While this is not an inherently sociotechnical problem, it has lightweight sociotechnical solutions. This participant noted that universities could have online documentation of which advisors are recruiting and what they are looking for.


